A Cubic-regularized Policy Newton Algorithm for Reinforcement Learning

We consider the problem of control in the setting of reinforcement learning (RL), where model information is not available. Policy gradient algorithms are a popular solution approach for this problem and are usually shown to converge to a stationary point of the value function. In this paper, we propose two policy Newton algorithms that incorporate cubic regularization. Both algorithms employ the likelihood ratio method to form estimates of the gradient and Hessian of the value function using sample trajectories. The first algorithm requires an exact solution of the cubic regularized problem in each iteration, while the second algorithm employs an efficient gradient descent-based approximation to the cubic regularized problem. We establish convergence of our proposed algorithms to a second-order stationary point (SOSP) of the value function, which results in the avoidance of traps in the form of saddle points. In particular, the sample complexity of our algorithms to find an $\epsilon$-SOSP is $O(\epsilon^{-3.5})$, which is an improvement over the state-of-the-art sample complexity of $O(\epsilon^{-4.5})$.

==> arxiv/proofsketch.tex <==
\subsection{Proof of Theorem \ref{thm:cubRegNewtonBound}}
\label{pf-cubRegNewtonBound}
\begin{proof} \textit{(Sketch)}
The policy parameter $\{ \theta_k \}$ generated by Algorithm \ref{alg:policyNewton} will satisfy the following conditions .\footnote{For detailed proof of \eqref{param_lhs} and \eqref{param_rhs} check Lemma 6 and Lemma 7 of appendix B.1 in supplementary material.} where $\delta_k^g, \delta_k^{\Hess} > 0$ are the variance upper bound of estimated gradient and Hessian respectively
\begin{align}\label{param_lhs}
    &\sqrt{\E{\norm{\theta_k\! - \!\theta_{k-1}}^2}} \!
    \ge\!\max \left\{ A(\theta), B(\theta)
    \right\} ,\textrm{ where }\\
    &A(\theta) = \sqrt{\frac{\E{\norm{\nabla J(\theta_k)}} \!-\! \delta_k^g -\delta_k^{\Hess}}{L_{\Hess}\! +\! \alpha_K}} \textrm{ , and }B(\theta)\! =\! \frac{-2}{\alpha_k\! +\! 2 L_{\Hess}}\! \left[ \!\E{\lambda_{\min} \left( \nabla^2 J(\theta_k)\right)}\!\! +\!\! \sqrt{2(\alpha_k \!+\! L_{\Hess}) \!\delta^{\Hess}_k} \right]
\end{align}
and
\begin{equation}
\label{param_rhs}
\begin{split}
      \E{\norm{\theta_R - \theta_{R-1}}^3} 
    &\le \frac{36}{\sum_{k=1}^N \alpha_k} \bigg[  J(\theta_{0})\!  -\!  J^* \! +\!  \sum_{k=1}^N \frac{4 \left( \delta_k^g \right)^\frac{3}{2}}{\sqrt{3 \alpha_k}}+ \sum_{k=1}^N \! \left( \! \frac{18\sqrt[4]{2}}{\alpha_k} \right)^2\! \! \left( (L_{\Hess}\! +\! \alpha_k) \delta^{\Hess}_k \! \right)^{\frac{3}{2}} \bigg] ,
\end{split}
\end{equation}
where $\theta_R$ represents the final output of Algorithm \ref{alg:policyNewton}.
By choice of parameters mentioned in \eqref{params} and \eqref{param_rhs} we can ensure that
\begin{align*}
    \E{\norm{\theta_R - \theta_{R-1}}^3} &\le \frac{c \epsilon^{\frac{3}{2}}}{L_{\Hess}^{\frac{3}{2}}} .
\end{align*}
On the other hand, by \eqref{param_lhs} we can obtain
\begin{align*}
    \sqrt{\E{\norm{\nabla J(\theta_k)}}} \le (c^{1/3}+1) \sqrt{\epsilon} \textrm{ and } \frac{\E{-\lambda_{\min} \left( \nabla^2 J(\theta_k) \right)}}{\sqrt{L_{\Hess}}} \le (c^{1/3}+1) \sqrt{\epsilon},
\end{align*}
from which one can get \eqref{main}.

\end{proof}
\subsection{Proof of Theorem \ref{thm:approxNewtonBound}}\label{pf-approxNewtonBound}
The main claim of Theorem \ref{thm:approxNewtonBound} would follow from Theorem 1 of  \cite{jordan2018stochastic}, provided we verify Assumptions 1 and 2 from the aforementioned reference. For the sake of completeness, we state these assumptions and Theorem 1 of \cite{jordan2018stochastic} below.\\
\textbf{Assumption 1}: The function $J$ has the following property,
\begin{itemize}
    \item $l$-Lipschitz gradients: for all $\theta_1$ and $\theta_2$, $\norm{\nabla J(\theta_1)- \nabla J(\theta_2)}\leq l\norm{\theta_1-\theta_2}$.
    \item $\rho$-Lipschitz Hessians: for all $\theta_1$ and $\theta_2$, $\norm{\nabla^2 J(\theta_1)- \nabla^2 J(\theta_2)}\leq \rho\norm{\theta_1-\theta_2}$.
\end{itemize}
\textbf{Assumption 2}: $g(\theta;\tau)$ and $\Hess(\theta;\tau)$ should follow almost surely,
\begin{align*}
		&\mathbb{E}\!\norm{g(\theta ; \tau)\!-\!\nabla \!J(\theta)}^2 \!\le M_1^2\textit{, } \norm{g(\theta ; \tau)\!-\!\nabla J(\theta)} \le M_1\textit{ and},
		\\
		&\mathbb{E}\!\norm{\Hess(\theta ; \tau)\!-\!\nabla^2 \!J(\theta)}^2 \!\le\! M_2^2\textit{, }\norm{\Hess(\theta ; \tau)\!-\!\nabla^2\! J(\theta)} \le M_2
	\end{align*}
\textbf{Theorem 1}: 
Let $J(\theta)$ satisfy the above Assumption 1, 2  and Algorithm \ref{algorithm 3} satisfies condition \ref{optimal_condition 1}, \ref{optimal_condition 2} with a pre-specified absolute constant $c$,
 $m_k\geq\max(\frac{M_1}{c_1\epsilon},\frac{\sigma_1^2}{c_1^2\epsilon^2})\log\Big(\frac{d \sqrt{\rho}}{\epsilon^{1.5}\delta' c}\Big)$ and $b_k\geq\max(\frac{M_2}{c\sqrt{\rho\epsilon}},\frac{\sigma_2^2}{c^2\rho\epsilon})\log\Big(\frac{d \sqrt{\rho}}{\epsilon^{1.5}\delta' c}\Big)\textit{ then }\forall\delta'\geq0 $, Algorithm \ref{alg:approx_policyNewton} will output an $\epsilon-$SOSP of $J$ with probability at least $1-\delta'$ within
 \begin{equation}
     O\bigg(\frac{\sqrt{\rho}\chi}{\epsilon^{1.5}}\bigg(\max\bigg(\frac{M_1}{\epsilon},\frac{M_1^2}{\epsilon^2}\bigg)+\max\bigg(\frac{M_2}{\sqrt{\rho\epsilon}},\frac{M_2^2}{\rho\epsilon}\bigg)\mathbb{T}(\epsilon)\bigg)\bigg)
 \end{equation}
total stochastic gradient and Hessian-vector product where $\chi\geq J(\theta_0)-J^*.$
\begin{proof}(\textbf{\textit{Theorem \ref{thm:approxNewtonBound}}})
    This proof can be directly concluded from Theorem 1 of  \cite{jordan2018stochastic} if assumption 1 and assumption 2 of \cite{jordan2018stochastic} mentioned above, hold true in our case.\\
From Proposition \ref{lipschitz-prop}, we can verify that assumption 1 of \cite{jordan2018stochastic} holds true and Lemma \ref{lemma:gradHessBounds} implies Assumption 2 of \cite{jordan2018stochastic}. Thus by the same logic from \cite{jordan2018stochastic}, we can conclude that  Algorithm \ref{alg:approx_policyNewton} will converge to an $\epsilon$-SOSP with probability $1-\delta$.
\end{proof}

\subsection{Proof of Corollary \ref{sample complexity}}\label{pf-samplecomplexity}
\begin{proof} \textit{(Sketch)}
Note that at each outer iteration we require  $m_k\geq\max(\frac{M_1}{c_1\epsilon},\frac{M_1^2}{c_1^2\epsilon^2})\frac{8}{3}\log\Big(\frac{2d }{\delta'}\Big)$ ,  $b_k\geq\max(\frac{M_2}{c_2\sqrt{\rho\epsilon}},\frac{M_2^2}{c_2^2\rho\epsilon})\frac{8}{3}\log\Big(\frac{2d }{\delta'}\Big)$ samples to approximate gradient and Hessian vector product respectively with probability $\delta'$
% with $\delta'=\frac{\delta}{3K_{out}}$ 
to control the total failure probability of Algorithm \ref{alg:approx_policyNewton}. From Theorem \ref{thm:approxNewtonBound} we have maximum number of iterations are $\Big[\frac{\sqrt{\rho}(J(\theta_0)-J^*)}{c\epsilon^{1.5}}\Big]$ and the inner complexity of Algorithm \ref{algorithm 3} is $\mathbb{T}(\epsilon)$. Furthermore by Lemma 2 of \cite{jordan2018stochastic} we have $\mathbf{T}(\epsilon)\leq O(\frac{1}{\sqrt{\epsilon}})$. Thus the gradient complexity becomes,
\begin{equation*}
\begin{split}
    S_G&\approx\frac{\sqrt{\rho}(J(\theta_0)\!-\!J^*)}{\epsilon^{1.5}}\!\times \max(\frac{M_1}{c_1\epsilon},\frac{M_1^2}{c_1^2\epsilon^2})\log\Big(\frac{2d}{\delta'}\Big)\\ 
    &\approx O(\frac{\sqrt{\rho}\sigma_1^2(J(\theta_0)-J^*)}{\epsilon^{3.5}})\textrm{ for } \epsilon\leq\frac{M_1^2}{c_1M_1}.
\end{split}
\end{equation*}
The total sample complexity of Hessian-vector product evaluation is 
\begin{equation*}
\begin{split}
    S_H \!&\approx\!\mathbb{T}(\epsilon)\!\!\times\!\!\frac{c\sqrt{\rho}(J(\theta_0)\!-\!J^*)}{\epsilon^{1.5}}\!\!\times\!\! \max(\frac{M_2}{c_2\sqrt{\rho\epsilon}}\!,\!\frac{M_2^2}{c_2^2\rho\epsilon})\frac{8}{3}\!\log\!\Big(\frac{2d }{\delta'}\Big)\\
    &\approx O(\frac{M_2^2(J(\theta_0)-J^*)}{\sqrt{\rho}\epsilon^{3}})\textrm{ for } \epsilon\leq\frac{M_2^4}{c_2^2M_2^2\rho}.
\end{split}
\end{equation*}
\end{proof}

